Geometry-Aware Planar Embedding of Treelike Structures

The growing complexity of spatial and structural information in 3D data makes data inspection and visualization a challenging task. We describe a method to create a planar embedding of 3D treelike structures using their skeleton representations. Our method maintains the original geometry, without overlaps, to the best extent possible, allowing exploration of the topology within a single view. We present a novel camera view generation method which maximizes the visible geometric attributes (segment shape and relative placement between segments). Camera views are created for individual segments and are used to determine local bending angles at each node by projecting them to 2D. The final embedding is generated by minimizing an energy function (the weights of which are user adjustable) based on branch length and the 2D angles, while avoiding intersections. The user can also interactively modify segment placement within the 2D embedding, and the overall embedding will update accordingly. A global to local interactive exploration is provided using hierarchical camera views that are created for subtrees within the structure. We evaluate our method both qualitatively and quantitatively and demonstrate our results by constructing planar visualizations of line data (traced neurons) and volume data (CT vascular and bronchial data

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> alg.tex <==

\Peggynote{Our novelties:
(1) hierarchical views for geometry information preservation
(2) effiecient and effective planarembedding
(3) exploration in 3D
(4) User interaction
}
An overview of our pipeline is shown in Fig.~\ref{fig:pipeline}.

When investigating a treelike structure, researchers are usually interested in the shape of the each tree segment (i.e., the angle between adjacent segments and length of segments).
However, it is challenging to observe the shape of a 3D treelike structure as a rendered result because of in-between segment occlusion in the skeleton projection and the loss of the structure information along the depth.(i.e., the third dimension in space beyond the 2D projection).
To overcome the segment occlusion in the rendered skeleton projection, our method generates an occlusion-free planar embedding for the original 3D skeleton while preserving the geometry attributes of each segment as much as possible.
For the information of the original structure lost in the planar embedding, particularly the 3D adjacency of each segment, our method designs a camera motion sequence for users' navigations through the original structure based on geometry information entropy rules.

Our method includes the optimal camera view finding for each bifurcation in the 3D structure in the pre-processing stage, and a dynamic planar embedding method in the real-time.
Specifically, in the pre-processing stage, we determine the optimal camera view for the nodes connected to each furcation node via maximizing the geometry information reflected on 2D view plane.
When the user triggers the planar embedding view generation, the planar visualization for the entire skeleton will be computed, combining both the hierarchical camera views computed in the pre-processing and the relative position between sibling nodes dependent on the user's viewpoint.
Beyond the planar visualization for the 3D skeletons, we developed a parallax-aware hierarchical navigation method for exploring the treelike structure in the original 3D space. A sequence of camera poses (i.e., view position and orientation) is generated by hierarchically connecting the optimal camera view for each subtree in the skeleton.
\Peggynote{
1. Arm issue;
2. Interaction, manual adjustment.
}
\subsection{Hierarchical View Finding}
\label{sec_hierView}
Our essential goal is to find the \emph{good} camera views for the input treelike structure.
This goal naturally leads to the question: what is the metric of camera view goodness for a treelike skeleton structure?
Treelike structures contain geometry information (for example, length, curvature, angle) and morphology information (for example, radius, branching frequency, adjacency).
Therefore, for our purpose, a good camera view should convey these information as much as possible. 
In this section, we present a quantitative metric for camera view goodness in neuron skeleton data and a fast camera view generation method for neuron data.

\subsubsection{Camera view metric}
We quantify the neuron information embedded in the neuron skeleton structures via Mutual Entropy \cite{Feixas2009Unified}.
%\cite{blahut1987principles}\cite{cover2012elements}.
\begin{equation}
I(v,O) = \sum_{o\in O} {p(o|v) \log \frac{p(o|v)}{p(o)}}
\label{eq:shannon_entropy}
\end{equation}
where $I(v,O)$ represents the information carried by the segment $o$ in the camera view $v$, probability of the occurrence of the corresponding neuron branch, and $\log p$ represents the information carried in this branch. In other words, \ref{eq:shannon_entropy} is to compute the sum of information expressed in the neuron skeleton in a certain camera view. In our method, $p = L_i/L_T$ where $L_i$ is i-th branch, and $L_T$ is the total length of all branches.

Unlike existing works that focused on viewpoint for mesh-based models, the geometry information reflected by skeleton data is quantified in segment length. However, the skeleton is not well-defined if only skeleton segments are recorded. We consider not only the real segments, but also the relative position between nodes and their siblings, the relative position between nodes and their parent's siblings as shown in Figure ~\ref{fig:additional_segmentconnect}.

\begin{figure}
    \centering
    \includegraphics[width=2in]{images/fig_skeleton.png}
    \caption{Mutual entropy in skeleton data. And the result with/without additional connections.}
    \label{fig:additional_segmentconnect}
\end{figure}

\subsubsection{Camera view hierarchy}
Given an arbitrary tree-like struture, geometry and morphology information are expanding through two phases in the visualization: the global view and detailed view.
We present a view hierarchy to include both the information in the best global view and that in a local view for fine structures.
The level of details is determined by the visible subtree level of a specific camera view.
To find the optimal camera view $v_Li$ for the subtree with the level $Li$ in the treelike structure, our objective function is
\begin{equation}
    E = \min_{v_{Li}}I(v_{Li},O_{Li})
\end{equation}
We denote the hierarchical viewpoint set for the tree structure as $$H=\{\{v_{Li}\}|\{v_{L0}\}, \{v_{L1_0}, v_{L1_1}, \cdots, v_{L1_{m1}}\}, \cdots, \{v_{Lh_0},v_{Lh_1},\cdots,v_{Lh_{mh}} \}\}$$
where $m1, m2, \cdots, mh$ represent the subtree amount in each tree level.
In Section \ref{alg:exploration}, a recommended exploration in 3D space will be generated based on this viewpoint set.

\subsection{Skeleton Planar visualization}
One of our main target is to unveal the hidden or invisible geometry information in 


\paragraph{Camera View Generation}


\input{orthographic_projection}

\textbf{Principle planes}
Given a 3D subtree structure $t_{Li_j}$, a primary view plane for this structure is defined as the plane passing the subtree center $C_{Li_j}$ and perpendicular with the direction of $v_{Li_j}$ where $j\in{0,1, \cdots, mi}$.

For each segment, we compute the furcation angle adjustment ratio $r_{furcation}$, within-chain angle adjustment ratio $r_{\theta}$ and length adjustment ratio $r_{length}$. 
The angle definition is shown in Figure \ref{fig:PSO_shaperecovery_angle}. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{images/parameterComparison.pdf}
    \caption{Curve placement with different parameters.}
    \label{fig:PSO_shaperecovery_angle}
\end{figure}

Each angle is bounded in $[0,\pi]$ so that the relative bending shape of each segment will be preserved in the planar embedding. 
We adopted PSO method to solve the skeleton shape recovery because the search space in this optimization problem is non-convex.

our current embedding result is shown in Figure \ref{fig:latest_result}. In our angle optimization method, we search for the optimal parameter combination. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=1.\linewidth]{images/segments.png}
%    \caption{Segment definition.}
%    \label{fig:PSO_shaperecovery_segment}
%\end{figure}

\begin{algorithm}[h]
\SetAlgoLined
\KwResult{\{$r_{furcation}$\}, \{$r_{\theta}$\}, and \{$r_{length}$\}}
 Init: \{particles\}\;
\While{Best Energy repeated for 20 times}{
    Calculate shape recovery result using each particle's ratio sets \{$r_{furcation}$\}, \{$r_{\theta}$\}, and \{$r_{length}$\} \;
    
    Compute Energy(planar embedding) using each particle's ratio set\;
    Update the best ratio set (of the minimal energy) among all particles\;
    Update the best ratio set (of the minimal energy) within each particle's history\;
    Update particle's ratio set for next loop\;
 }
 \caption{Shape recovery using particle swarm optimization}
 \label{alg:PSO_shaperecovery}
\end{algorithm}

\subsection{Exploration in 3D space}
\label{alg:exploration}
%We are inspired by the smooth camera motion generation method developed in \cite{lino2015intuitive}. 
It is inevitable that some spatial information is not fully rendered on the planar embedding while the treelike structure's node length, angle, and curvature information are well-preserved.
To complement the geometry information loss, we generate a camera motion that smoothly connects the hierarchical best views for each subtree in the skeletal structure.
Users explore the raw treelike structure in 3D space in each views that reveal the maximal information.
Furthermore, the tree levels of focus can be specified by users.
Based on Section \ref{sec_hierView}, a series of best views for demonstrating the geometry information in the original tree is generated.
We use a quadratic Bézier curve to connect adjacent views for the structure exploration.



==> introduction.tex <==
Parallel to humanity's constant endeavour to discover and learn about the structures and operations of things around us, humans have also introduced ways to abstract these discoveries in the form of simpler representations: 2D scene capture, cartography, wiring diagrams for electronic systems, skeletal representation of chemical bonds, genomics annotations, connectomics for mapping neuronal systems, to name but a  few.   
Specifically in the life sciences domain, recent advancements in image acquisition technology and techniques for 3D reconstruction and visualization~\cite{preim2016survey} have made it possible for scientists to study, at a greater degree, intricate and complex biological systems.
%Though the study of structures in 3D has proven to enhance understanding~[ref], however, hardware and equipment for 3D visualization is still a limited asset within the practical daily workflow of scientists.
%Moreover, as the morphology of a structure grows in complexity, its investigation becomes more challenging due to clutter, occlusions, and at times, inability to seamlessly manipulate camera orientations within the visualization application.
%Though the study of structures in 3D has proven to enhance understanding~[ref], however, as the morphology of a structure grows in complexity, its investigation becomes more challenging. %%%% could not find a reference to support 3D improves understanding statement
%
Though 3D representations can more accurately model spatial and structural information, however, as the morphology of a structure grows in complexity, its study in the 3D domain becomes more challenging. %%%% could not find a reference to support 3D improves understanding statement
This is primarily due to data density clutter and occlusions, and at times, inability to seamlessly manipulate camera orientations within the visualization application.
To this end, one solution has been to reduce the image-space dimensionality and visualize 3D structures in 2D.
%Therefore, the next logical step for an abstracted understanding of the 3D structures is its 2D representation.
%In doing so, it has been shown that for the 2D representation or planar visualization of data, it is important to maintain a sense of the morphology~\cite{borkin2011evaluation}.
In doing so, it has been shown that it is important to maintain a sense of the original morphology of the object when reconstructing its 2D representation or planar visualization~\cite{borkin2011evaluation}.
This not only ensures a better and a holistic understanding of the structure but also improves the accuracy and efficiency of carrying out certain tasks.

In this paper, we aim to solve the planar layout reconstruction of 3D tree-like objects.
Tree-like anatomies are a common occurrence in biomedicine and given their importance, there has been great effort to extract them~\cite{lo2012extraction} and to generate their planar visualizations [refs].
Such structures extend from a starting point, branch out in different directions, and do not contain cycles.
%In recent years, due to its importance in the biomedical field, there have been several approaches to generate planar visualizations of tree-like anatomical structures~[refs]. 
%The simplest 3D visual representation of a tree-like object can be considered a skeleton structure.
In its simplest visual form, a tree-like object can be represented as a skeleton.  
%Using the skeleton data, common planar representation techniques generate linear connectivity graphs~\cite{munzner2003treejuxtaposer,al2014neurolines} or produce spatially coherent embeddings.
\textcolor{red}{What are some uses for skeleton visualization?}

%Given a 3D skeleton of a tree-like structure, we present a novel algorithm that generates a planar layout, while minimizing visual occlusions, self-intersections, and maintaining the general geometric morphology of the original structure.
We present a novel algorithm that generates a planar layout of 3D tree-like skeletons, while minimizing visual occlusions, self-intersections, and maintaining the general geometric morphology of the original structure.
We achieve this by following three broad steps: (1) generating projection planes for each sub-tree segment of the 3D structure, (2) determining the 2D angles of the projected points, and (3) reconstructing a planar layout of the structure while maintaining the above mentioned properties. \textcolor{orange}{(need to confirm with Peggy).}
%We achieve this by first determining the projection planes for segments in the 3D structure that would best preserve their lengths and curvatures.
Existing techniques that utilize view-based projections for generating planar layouts require an input projection matrix that is applied globally to determine the geometric attributes for recovering the 2D shape of the 3D object \textcolor{red}{(need to make sure that this claim is accurate and no other works employ a sub-tree projection approach)}. 
This can be a very time consuming task if users are required to provide an appropriate global view.  %, specifically for complex structures.
Specifically, for a complex structure with extensive branching angles, it becomes exceedingly difficult to find a global projection plane which can best preserve each segment of the structure's shape and geometric attributes.
%To overcome these limitations, we employ a particle-swarm view-finding optimization approach to automatically determine projection planes for each sub-tree segment in the structure, based on mutual entropy \textcolor{orange}{(in? of?)} the data. %,
To overcome these limitations, in contrast to using a global projection, we iterate over the entire structure and automatically determine optimal projection planes using particle-swarm optimization~(PSO) [ref], for each subtree segment.
PSO is a computational technique that solves an objective function using a swarm of particles distributed in space that are guided towards a candidate solution with regard to a given measure of quality. 
The objective function we have designed aims to minimize the mutual entropy \textcolor{orange}{(in? of?)} the data...\textcolor{red}{Peggy, need to finish the sentence here.} %,using a particle-swarm based view-finding optimization function.
\textcolor{orange}{Some line about camera maneuvering in medical visualization...}
The view-point projections from this step is also utilized in our visualization application....
%To overcome this challenge, we introduce a particle-swarm based view-finding optimization function that given a collection of 3D points ....
%Moreover, [do not use a singular camera view, rather determine camera view for segments of the tree-like structure.]
%Next, we employ an energy function that generates a 2D layout of the entire structure that 
%A final 2D layout of the entire structure is generated using geometric properties determined from the projected segments, we employ an energy function that preserves the geometric attributes of the segments while avoiding self-intersections.

For the final shape reconstruction, we have designed an energy function that aims to preserve the geometric attributes of the projected segments while minimizing self-intersections in the overall 2D layout.
%To reconstruct a 2D layout of the entire structure is generated using an energy function that preserves the geometric attributes of the projected segments while minimizing self-intersections.
A complete 3D tree-like object can have a diverse range of geometric morphologies within its structure and naturally, in reducing the dimensionality to 2D, it is not be possible to perfectly preserve all shape attributes.
However, we leverage an assumption that a domain expert user may have certain preferences based on the purpose of the embedding reconstruction and given the nature of the data.
That is to say, one may want to study the overall curvature and shape of the object and may not require the accurate reconstruction of the angular values, for instance.    
To this end, we enable users to relax or enforce \textcolor{orange}{length, curvature, and ...?} attributes based on their preferences.
Moreover, our visualization application also allows users to interactively refine embedding layouts by dragging nodes in the 2D space and recalculating the layout generation based on the user-defined adjustment.  
 

% \textcolor{red}{ 
% - Curved Planar Representation + other spatially-coherent techniques require input parameters that are used a global embedding rule\\
% - One rule does not fit all + user cannot try different embedding techniques for different complexities\\
% - users may have different choice for relaxing rules (any evidence / example? any advantage?\\
% - Therefore, we introduce a novel planar embedding technique that uses user input preference as a weight and apply those to find the best planar views in a coarse-to-fine model.\\
% - Moreover, our visualization application allows users to interactively fix and update the embedding result. }






We summarize our contribution as follows:
\begin{itemize}
    \item Developing an interactive planar visualization method for treelike medical data to achieve an occlusion-free planar view while preserving the geometry information (i.e., the node angles and edge lengths) in the treelike structures.
    \item Providing a hierarchical navigation using our information-entropy-based view finding method.
    \item A user interface enabling users to extract the planar visualization and hierarchical navigation based on customized requirement or research interest.
\end{itemize}

==> introduction_v2.tex <==
%Treelike anatomical objects are a common occurrence in biological systems and their visualization is of great importance, especially when analyzing structures belonging to the respiratory, vascular, and nervous systems.
%This paper describes an algorithm for generating a planar embedding map for 3D treelike structures, by presenting the branches of the structure in a single view while minimizing
%%
Many critical biological systems, such as the vascular, respiratory, and nervous system, consist of structures that express a treelike topology.
%Recent advancements in image acquisition technology and techniques for 3D reconstruction and visualization~\cite{preim2016survey} have made it possible for scientists to observe, at a greater degree, these intricate and complex systems.
%Recent advancements in image acquisition technology have made it possible to capture, at a finer scale, these intricate and complex systems and coupled with techniques for 3D reconstruction and visualization~\cite{preim2016survey}, domain scientists are able to examine, at a greater degree, the topology of these structures [ref skeletonization, neuron tracing, connectomics, etc], such as its external geometry, branching pattern and curvature, and internal flow capacity.
Recent advancements in image acquisition technology coupled with techniques for 3D reconstruction and visualization~\cite{preim2016survey}, have enabled domain scientists to examine, at a finer scale, attributes of these intricate and complex structures [ref skeletonization, neuron tracing, connectomics, etc], such as their external geometry, branching pattern, curvature, and internal flow capacity.
%Depending on the domain of investigation, experts need to study the external topology of these structures [ref skeletonization, neuron tracing, connectomics, etc], such as its overall shape, branching pattern and curvature, or observe its tubular-shaped interior [ref virtual endoscopy, vc, etc.].
%Though inspecting objects in 3D can more accurately present spatial and structural information, however, as the  morphology of a structure grows in complexity, its investigation in the 3D domain becomes more challenging. %%%% could not find a reference to support 3D improves understanding statement
Though inspecting objects in 3D can more accurately present spatial and structural information, however, as the branching morphology grows in complexity, its investigation in 3D space becomes more challenging.
This is primarily due to data density clutter, visual occlusions, and at times, the inability to seamlessly manipulate camera orientations within the visualization application to thoroughly explore the data.
Due to this, domain scientists often prefer to visualize relevant structures and branches of an anatomy in a single schematic view, similar to their common practice of hand-drawing a representation of the anatomy they wish to convey or report~\cite{won2009uncluttered}.
To this end, planar visualization techniques have been introduced that aim to reduce the complexity of viewing 3D data by solving its appropriate embedding in 2D space.
In doing so, it has been shown that to ensure a holistic understanding of the structure, the 2D representation must maintain a sense of the original 3D morphology~\cite{borkin2011evaluation}.
Moreover, specific to treelike objects, it is also important that the generated planar views correctly reveal the relevant branches and avoid misleading distortions and overlaps which, as a result, could hamper the reader's recognition of the anatomy.
These challenges and requirements have motivated us to develop a method for the planar visualization of the topology of treelike objects, that preserves, to the best possible extent, the geometric morphology of the original structure and minimizes self-intersections.
%While our algorithm is general for any treelike object, \textcolor{orange}{NAME} was designed as a solution to visualize topologies of neuronal \textcolor{orange}{(and vascular?)} structures. 


%Due to these challenges, domain scientists have often preferred visualizing branching anatomies in a single schematic view, analogous to their common practice of hand-drawing representations ~\cite{won2012uncluttered}.
%
%To this end, we present a method for reconstructing a planar visualization of the topology of treelike objects, while minimizing self-intersections and preserving, to best possible extent, the topology of the original structure.
%Such a preference can be seen in the common practice by experts to hand-draw representations of the anatomy that they wish to convey or report.
%To this end, one solution has been to reduce the dimensionality of the image-space and visualize 3D structures in 2D.
%These challenges and requirements motivated us to develop \textcolor{orange}{NAME}, a method for reconstructing a planar visualization of the topology of 3D treelike objects.
%
%To address these challenges and requirements, planar visualization techniques have been introduced that reconstruct schematic representations of 3D data, such that users are able investigate its required extents without having to apply viewing transformations (apart from linear pan and zoom).
%Planar visualization techniques aim to reduce the complexity of viewing 3D data by projecting it onto 2D space.
%This allows user to investigate the required extents of the data without having to rotate the data in an attempt t
%However, in doing so, it has been shown that the 2D representation must maintain a sense of the original 3D morphology~\cite{borkin2011evaluation}.
%This not only ensures a better and a holistic understanding of the structure but also improves the accuracy and efficiency of carrying out certain tasks.
%To ensure a holistic understanding of the structure, it has been shown that the 2D representation must maintain a sense of the original 3D morphology~\cite{borkin2011evaluation}.
%This not only ensures a better and a holistic understanding of the structure but also improves the accuracy and efficiency of carrying out certain tasks.
%Moreover, specific to treelike objects, it is also important that the generated planar views correctly reveal as many of the relevant branches as possible, while avoid misleading overlaps that could hamper the reader's recognition of the anatomy.
%
%We define our 2D view reconstruction scheme by following three broad steps: (1) dividing the tree structure into segments and generating projection planes for each sub-tree segment, (2) determining 2D angles of the projected branches, and (3) reconstructing a 2D map of the topology while minimizing morphological distortion and avoiding branching overlaps.
We define our 2D-view reconstruction scheme by first dividing the tree into subtree segments, based on a defined branching morphology, and then projecting each segment onto a 2D plane to generating projection planes for each sub-tree segment and then using the projected morphology 
In its simplest visual form, a tree topology can be represented as a skeleton structure in which nodes are positioned at points where there is a change in morphology (such as bends or branching points) and edges, shown as lines, connecting these nodes (see Fig.XX).   
Due to the importance of visualizing treelike objects in life sciences, there exists a great deal of work to extract skeletons based centerline computation or \textcolor{orange}{other?} 
Given a 3D skeleton, we define our planar embedding algorithm to maintain the geometric context of the original structure by preserving the length and bending angles of the skeleton structure. 

%we reconstruct a 2D view following three broad steps: (1) dividing the tree structure into segments and generating projection planes for each sub-tree segment, (2) determining 2D angles of the projected branches, and (3) reconstructing a 2D map of the topology while minimizing morphological distortion and avoiding branching overlaps.
 



%While our algorithm is general for any treelike structures, \textcolor{orange}{NAME} was designed as a solution to visualize topologies of neuronal \textcolor{orange}{(and vascular?)} structures. 
%
%Our planar embedding algorithm follows three broad steps: (1) generating projection planes for each sub-tree segment of the 3D structure, (2) determining the 2D angles of the projected points, and (3) reconstructing a planar layout of the structure while maintaining the above mentioned properties. \textcolor{orange}{(need to confirm with Peggy).}



%Additionally, these methods are used to facilitate effective visual comparisons by juxtaposing or overlaying the generated 2D layouts.
 


\textcolor{red}{Take aways from seminar meeting: \\
- Look at graph planarlization. Also try NOT to make it sound like a graph problem.\\
- no current work for best-view of skeleton structure. Current works aim for traingle projection.\\
- since simple line projection is not enough, mutual entropy enforces the capturing of spatial relationship}

==> introduction_v22.tex <==
Many critical biological systems, such as the vascular, respiratory, and nervous system, consist of structures that express a treelike topology.
Recent advancements in image acquisition technology coupled with techniques for 3D reconstruction and visualization~\cite{preim2016survey}, have enabled scientists to examine, at a finer scale, the attributes of these intricate structures [ref skeletonization, neuron tracing, connectomics, etc], such as their external geometry, branching pattern, curvature, and flow capacity.
Though spatial and structural information can be more accurately presented in 3D, however, as the branching morphology of an object grows in complexity, its inspection becomes more challenging.
This is primarily due to data density clutter, visual occlusions, and at times, the inability to seamlessly manipulate camera orientations within the visualization application to thoroughly explore the data.
Due to these challenges, experts often prefer to visualize a schematic representation of the relevant branches of an object, in a single 2D image~\cite{won2009uncluttered}.
This has motivated us to develop a method to create planar embeddings of the topology of treelike structures, where there are minimal visual occlusions and the 2D layout preserves the geometric morphology of the original anatomy.

%Given the functional importance of treelike structures in medicine, there has been great effort in designing methods for their schematic representations~\cite{kreiser2018survey}.
%
Given the functional importance of treelike structures in medicine, there is often great effort in extracting them~\cite{lo2012extraction}.
A planar schematic image that presents all relevant branches of a structure in a single view and illustrates its topological attributes, can be very beneficial in clinical settings, specifically for reporting examinations and diagnosing abnormalities.
For instance, physicians are particularly careful about ensuring that they have observed the entire structure without missing any regions. 
A planar representation can be used as guidance map to track observation coverage or to facilitate a holistic understanding of a current local 3D view with respect to the entire structure.
Moreover, a single schematic image that captures complex anatomical and physiological information can be used for medical record keeping.
Rather than serving for primary interpretation, experts can utilize these images to effectively annotate and communicate key features with other collaborators or juxtapose with other records to track variations.
It has been indicated that to ensure the reader's recognition of the anatomy the planar embeddings should maintain a sense of the geometric context of the original structure and the branches should avoid misleading overlaps and have minimal distortion.

In this work, we utilize the 3D skeleton of a treelike structure, typically extracted using centerline computation or \textcolor{orange}{other?}, as the topological outline for producing a map of the underlying anatomy.
One key characteristic of geometrically-coherent planar visualization methods~\cite{marino2015planar,won2012uncluttered} is that they use a fixed global view by which to map the 3D anatomy.
In contrast, we construct our planar layout by first dividing the anatomy into subtree segments based on a defined branching order, and then generating projection planes for each segment to determine subtree-specific planar geometric attributes.
To this end, the first novel contribution of this paper is our projection plane calculation algorithm. 
Projecting a collection of 3D lines onto 2D requires a set of preservation attributes to be defined in order to maintain the original geometric morphology of the anatomy. 
This could be the line length or bending angles.
Beyond the two attributes, we have additionally designed a mutual-entropy functiont hat checks for the spatial relationship of a node in the skeleton with respect to its linked surrounding nodes. 
Naturally, reducing the dimensionality of data means loss of one or more attributes, and therefore it is not possible to accurately preserve all attributes. 
To compute the best projection plane, we employ particle swarm optimization (PSO).
PSO is a computational technique that solves an objective function using a swarm of particles distributed in space that are guided towards a candidate solution with regard to a given measure of quality. 
Therefore, to determine a projection plane for a set of branches, our objective function minimizes mutual entropy, and maximizes the preservation of branch length. 

Using 2D bending angles calculated for each projected branch, we then embed the geometric attributes to the 2D map while avoiding branching intersections.
To achieve this, we again deploy a PSO 




%While most existing techniques present methods for flattening the interior or exterior surfaces of an object, in a linear fashion~\cite{kreiser2018survey},  our embedding algorithm 
Given a 3D skeleton, we define our planar embedding algorithm to maintain the geometric context of the original structure by preserving the length and bending angles of the skeleton structure. 
 


\textcolor{red}{Take aways from seminar meeting: \\
- Look at graph planarlization. Also try NOT to make it sound like a graph problem.\\
- no current work for best-view of skeleton structure. Current works aim for traingle projection.\\
- since simple line projection is not enough, mutual entropy enforces the capturing of spatial relationship}

==> macro.tex <==

\definecolor{TodoColor}{rgb}{0,0.5,0} 

\newcommand{\notes}{1}

\ifthenelse{\equal{\notes}{1}}
{
    \newcommand{\Joenote}[1]{\textcolor{purple}{Joe:#1}}
    \newcommand{\Saeednote}[1]{\textcolor{orange}{Saeed:#1}}
    \newcommand{\Peggynote}[1]{\textcolor{TodoColor}{Peggy:#1}}
}
{
    \newcommand{\Peggynote}[1]{}
}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> results_old.tex <==
%In this section we present scenarios where our planar embedding can be utilized to facilitate scientific visualization.

Though our technique is general and can be applied to any treelike structure, we demonstrate our work using traced neuronal data and segmented vascular and bronchial data.

\Joenote{Paragraph about the datasets used.}

\Joenote{Paragraph about the general embedding results in Fig. 6 (not really visualization).}

\Joenote{\textbf{Planar Visualization.}}

\Joenote{Paragraph about guidance map.}

\Joenote{Paragraph about rendering surface using radius values.}

\Joenote{Paragraph about juxtaposition.}

\Joenote{\textbf{Navigation Camera Path.}}

\Joenote{Paragraph about exploration.}

\Joenote{\textbf{Performance.}}

\Joenote{Paragraph about performance numbers and table.}

\Joenote{OLD REMAINDER STUFF BELOW:}

Though our technique is general and can be applied to any treelike structure, we demonstrate our work using traced neuronal data and segmented vascular and bronchial data.
To \textcolor{red}{qualitatively} \Joenote{I'm not sure if we need to keep using the word 'qualitatively'.} evaluate our results, we show the reconstructed planar embedding along with separate 3D views for comparison.
For tasks that require direct inspection of the object, we show how planar visualization of cranial blood vessels can help detect abnormalities, such as vascular aneurysm, in a single view. 
Current research in neuroscience is actively engaged in mapping the connectivity of the brain to identify structural degeneration that leads to brain diseases.
To this end, we show how the planar visualization of olfactory neurons can help scientists study fragmentation patterns.
Next, we demonstrate the effectiveness of our generated camera path to facilitate exploration of treelike objects in the volume.
Finally, we report memory and computation time performance of our algorithm \textcolor{orange}{and compare it with similar planar visualization works.}

\paragraph{\textbf{Planar Visualization.}}
Figure~\ref{fig:results} shows the results of our planar embedding algorithm using skeletons of five different datasets: two olfactory neuron data from the DIADEM dataset~\cite{brown2011diadem}, and two blood vessels (aorta and lower limb). \Joenote{This is 4, will the bronchial tree be number 5?}.
The skeletons for the neuron datasets are extracted using gold-standard neuron tracing algorithms, provided with the dataset, and the skeletons for the blood vessels are computed using~\cite{bitter:2001:tvcg}.
\textcolor{orange}{To qualitatively evaluate our result, we also show two independent 3D views of the original input skeleton.} \Joenote{Again, probably don't need to say 'qualitatively'.}
From the 3D view points it can be observed that simplistic orthogonal or perspective projections that display 3D branching structures on a 2D screen, distort the morphology of the branches that have different principal axes or often causes false intersections of branches that can mislead the reader’s recognition of the structure.
Therefore, our embedding results are able to preserve the global shape of the object while also reflecting the local geometry of individual branches \textcolor{purple}{I feel like I have used this statement over a 1000 times!!}. 
 


One important utility of planar visualization is to use it as a guidance map that can aid domain users to investigate attributes of the data using a single schematic view.
Particularly for non-invasive clinical diagnosis, physicians require methods to expedite anomaly detection, to accommodate large volumes of patient scans, while also being careful not to miss a region within the data~\cite{park2019cmed}.
Here, we show an example of aneurysm detection (bulge or ballooning of a vessel) in cranial blood vessels using a visualization generated from our embedding technique. \Joenote{Not sure if we should really call it aneurysm detection, as then we would need to evaluate how accurate it is.}
Fig.~\ref{fig:teaser}(a) shows a surface rendering of segmented blood vessels from a CT scan.
The color map\footnote{The diverging color map for three classes was designed using ColorBrewer~\cite{harrower2003colorbrewer} (\url{https://colorbrewer2.org/}) with the `color blind safe' and `print friendly' options.} represents the gradient of the radii difference of a segment with respect to the average radius of the entire structure, where the colors are mapped from a shade of blue to yellow to red, in order of increasing segment radius value. 
Though the 3D rendering already provides a better view than scrolling through slices of the CT scan, a radiologist is still required to manipulate camera views within the visualization application to detect the bulged vessel and simultaneously take a mental note of the radii.
In contrast, using a planar visualization as in Fig.~\ref{fig:teaser}(b), a radiologist is able to visualize all the blood vessels and compare their geometric attribute (i.e., radius) within a single view. 
Moreover, there are two additional advantages to such a visualization.
Firstly, it has been shown that 2D representation of medical data helps carry out tasks more effectively~\cite{borkin2011evaluation} and therefore, by preserving the global shape of the original structure, a domain expert can more efficiently navigate the 3D structure to confirm the findings from the planar view.
Secondly, by preserving the shape, domain scientists can present the representation to collaborators who will be able to recognize the anatomy. \Joenote{Should some if this be in discussion instead of the results (hypothesizing on how to use, etc.?). Also, we might want to keep more general in nature (e.g., just say what is showed in terms of mapping color, user (instead of radiologist) can observe, etc.)  I'm concerned there is a larger chance the reviewers will ask for domain feedback if we give such a specific application.}

Connectomics~\cite{TheHumanConnectome} is an emerging field of techniques and frameworks for the study of complex neural connection maps.
Insights gained from these tools are being applied to understand how the human brain functions and eventually, analyze the degradation process as a result of cognitive decline or diseases. 
A common challenge address by researchers is the immensity of volume data, captured using micro- and nano-resolution imaging technologies. 
Recent works~\cite{mohammed2017abstractocyte,al2014neurolines} have introduced methods to alternatively represent dense neuronal structures as abstracted diagrams, albeit in a linear graph-like arrangement.
%In , we demonstrate the utility of our planar embedding technique for studying patterns in neurodegeneration.
%A utility of our planar embedding technique for studying patterns in neurodegeneration is demonstrated in Fig.~\ref{fig:juxtapose}.
Though schematic diagrams have proven to be very helpful in studying connections and their topological layout, however, an examination of the structure is required to understand morphological changes during degeneration. 
%Inspecting a neuronal structure in a dense volume is a time-consuming task and therefore, neuroscientists usually rely on population analysis for designing their hypothesis. 
To this end, we propose a planar visualization approach for studying the corresponding structural changes within a neuronal structure by juxtaposing the projected structures in a single view.
We demonstrate this idea in Fig.~\ref{fig:juxtapose}, using an isolated olfactory neuron (Fig.~\ref{fig:juxtapose}(b)) from a dense brain microscopy volume (Fig.~\ref{fig:juxtapose}(a)), its corresponding \textit{diseased} state (Fig.~\ref{fig:juxtapose}(c)), and its skeleton representation.
First, we construct a planar embedding of the neuron's skeleton data (Fig.~\ref{fig:juxtapose}(d)), using our method.
Next, we generate a volume rendering of the 3D structure using a view point perpendicular to the central axis of the skeleton and project it onto a single view based on the embedding result. 
Since the \textit{diseased} neuronal structure is fragmented and hence, not a \textit{single} tree object, we use the 3D skeleton from (a) to segment and embed the neuron. 
Finally, we juxtapose  the two embedded volumes in a single view with an offset for clarity, as shown in Fig.~\ref{fig:juxtapose}(e).
Thus, using this method, neuroscientists can effectively analyze fragmentation and thinning patterns within a neuron. \Joenote{Again, not sure if this is more discussion.}



%\textcolor{red}{Neuroscientists can analyze fragmentation and thinning patterns by juxtaposing the \textit{healthy} and \textit{disease} neurites, as shown in (e), instead of separately studying them in 3D.} \Joenote{This probably belongs more in the paper text than the caption (still with direct reference to subfig (e)).}



\paragraph{\textbf{Navigation Camera Path.}}
To investigate a 3D object, one of the most natural way is to freely explore the information in the 3D space.
With this motivation, our technique generates a camera path with dynamic focus on the different subtrees in the skeleton for users to explore the original 3D data in representative views.
This camera path is to show the structure in a top-down way, starting with the global best view and then navigate through each representative view of each subtree.
A spherical dolly motion around each subtree makes use of parallax to aid in understanding the geometry information along the view depth direction.
A smooth transition between two views builds up a perception of spatial relationship between different parts in the structure.
\textcolor{red}{Figure X} shows the hierarchical views for the structure of lower limb vessels which includes four levels of hierarchical levels.
Each representative viewpoint focuses on different level of details of the structure.
Please refer to our supplementary video for a demonstration of our recommended exploration.

\subsection{Performance}
Time and Memory.
\input{tab_timecost}

==> userstudy.tex <==
\subsection{User study}

\Peggynote{

To evaluate the effectiveness of our embedding and exploration result, we conduct a user study on multiple datasets.
Dataset we are using include Hippocampal neuron1, Bronchial airways, and Cranial blood vessels.
To test various structure complexity, the three datasets are chosed based on their node numbers.
Functions:
\begin{itemize}
    \item Let users freely explore the Dataset A for 2 minutes. Alternative: Then show them exploration suggested by our method. After the exploration, show them two segments (one is original, one is in modified shape ) and ask them "Which one do you think is a segment in the original dataset?"
    \item Global view comparison: given Dataset A, starting with a random view, let the user freely explore the dataset for 2 minutes, then let them decide which view is the best view. Alternative: after 2 minute's exploration, show the global best view generated using our method and then show them with a randomly picked view. ``Which view is more representative in terms of showing geometry information of the dataset?''
\end{itemize}

Each subject has two trials.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.\linewidth]{user_study.PNG}
    \caption{User Study Pipeline.}
    \label{fig:userstudy}
\end{figure}

}


==> visual_comparison.tex <==
\begin{figure*}[t!]
\centering
\begin{minipage}[c]{\linewidth}

	\label{fig:aneurix}
	\includegraphics[width = \linewidth]{images/visualcomparison/aneurix.PNG}

\end{minipage}
\begin{minipage}[c]{\linewidth}

	\label{fig:aorta}
	\includegraphics[width = \linewidth]{images/visualcomparison/aorta_trial1.PNG}	

\end{minipage}
\begin{minipage}[c]{\linewidth}

	\label{fig:neuron1}
	\includegraphics[width = \linewidth]{images/visualcomparison/neuron1.PNG}	

\end{minipage}
\begin{minipage}[c]{\linewidth}

	\label{fig:neuron2}
	\includegraphics[width = \linewidth]{images/visualcomparison/neuron2.PNG}	

\end{minipage}
\Caption{Planar visualization of different treelike structures}
{%

}
\label{fig:evaluation_tile}
\end{figure*}

